StarryGazer: Leveraging Monocular Depth Estimation Models for Domain-Agnostic Single Depth Image Completion

The problem of depth completion involves predicting a dense depth image from a single sparse depth map and an RGB image. Unsupervised depth completion methods have been proposed for various datasets where ground truth depth data is unavailable and supervised methods cannot be applied. However, these models require auxiliary data to estimate depth values, which is far from real scenarios. Monocular depth estimation (MDE) models can produce a plausible relative depth map from a single image, but there is no work to properly combine the sparse depth map with MDE for depth completion; a simple affine transformation to the depth map will yield a high error since MDE are inaccurate at estimating depth difference between objects. We introduce StarryGazer, a domain-agnostic framework that predicts dense depth images from a single sparse depth image and an RGB image without relying on ground-truth depth by leveraging the power of large MDE models. First, we employ a pre-trained MDE model to produce relative depth images. These images are segmented and randomly rescaled to form synthetic pairs for dense pseudo-ground truth and corresponding sparse depths. A refinement network is trained with the synthetic pairs, incorporating the relative depth maps and RGB images to improve the model's accuracy and robustness. StarryGazer shows superior results over existing unsupervised methods and transformed MDE results on various datasets, demonstrating that our framework exploits the power of MDE models while appropriately fixing errors using sparse depth information.

==> figures/Overview.tex <==
\begin{figure}[t]
   \centering
    \includegraphics[width=\linewidth]{figure_assets/Overview.pdf}
    \caption{\textbf{Sparse depth image~(Top). Depth image completed by StarryGazer~(Bottom).}}
    \label{fig:overview}
\end{figure}

==> figures/noise_qual.tex <==
% \documentclass{article}  % or any other class you are using


\begin{figure}[h]
     \centering
     \begin{subfigure}[b]{0.11\textwidth}  
         \centering
         \includegraphics[width=\textwidth, page=10]{figure_assets/noise_qual.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.11\textwidth}  
         \centering
         \includegraphics[width=\textwidth, page=3]{figure_assets/noise_qual.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.11\textwidth}  
         \centering
         \includegraphics[width=\textwidth, page=2]{figure_assets/noise_qual.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.11\textwidth}  
         \centering
         \includegraphics[width=\textwidth, page=1]{figure_assets/noise_qual.pdf}
     \end{subfigure}
     \hfill     
     \begin{subfigure}[b]{0.11\textwidth}  
         \centering
         \includegraphics[width=\textwidth, page=11]{figure_assets/noise_qual.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.11\textwidth}  
         \centering
         \includegraphics[width=\textwidth, page=6]{figure_assets/noise_qual.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.11\textwidth}  
         \centering
         \includegraphics[width=\textwidth, page=5]{figure_assets/noise_qual.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.11\textwidth}  
         \centering
         \includegraphics[width=\textwidth, page=4]{figure_assets/noise_qual.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.11\textwidth}   
         \centering
         \includegraphics[width=\textwidth, page=12]{figure_assets/noise_qual.pdf}
         \caption*{$\sigma$ = 0}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.11\textwidth}  
         \centering
         \includegraphics[width=\textwidth, page=9]{figure_assets/noise_qual.pdf}
         \caption*{$\sigma$ = 0.001}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.11\textwidth}  
         \centering
         \includegraphics[width=\textwidth, page=8]{figure_assets/noise_qual.pdf}
         \caption*{$\sigma$ = 0.01}  
     \end{subfigure}   
     \hfill
     \begin{subfigure}[b]{0.11\textwidth}  
         \centering
         \includegraphics[width=\textwidth, page=7]{figure_assets/noise_qual.pdf}
         \caption*{$\sigma$ = 0.1}
     \end{subfigure}
        \caption{
        Qualitative comparison on NYU Depth V2 dataset. 
        }
        \label{fig:noise_qual}
\end{figure}


==> figures/segment_qual.tex <==
\begin{figure}[h]
     \centering
     % Second Row
     \hfill 
     \begin{subfigure}[b]{0.11\textwidth}  
         \centering
         \includegraphics[width=\textwidth, page=1]{figure_assets/segment_qual.pdf}
     \end{subfigure}
     \hfill     
     \begin{subfigure}[b]{0.11\textwidth}  
         \centering
         \includegraphics[width=\textwidth, page=7]{figure_assets/segment_qual.pdf}
     \end{subfigure}     
     \hfill   
     \begin{subfigure}[b]{0.11\textwidth}  
         \centering
         \includegraphics[width=\textwidth, page=10]{figure_assets/segment_qual.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.11\textwidth}  
         \centering
         \includegraphics[width=\textwidth, page=4]{figure_assets/segment_qual.pdf}
     \end{subfigure}
     % Third Row
     \begin{subfigure}[b]{0.11\textwidth}  
         \centering
         \includegraphics[width=\textwidth, page=2]{figure_assets/segment_qual.pdf}
     \end{subfigure}
     \hfill     
     \begin{subfigure}[b]{0.11\textwidth}  
         \centering
         \includegraphics[width=\textwidth, page=8]{figure_assets/segment_qual.pdf}
     \end{subfigure}
     \hfill     
     \begin{subfigure}[b]{0.11\textwidth}  
         \centering
         \includegraphics[width=\textwidth, page=11]{figure_assets/segment_qual.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.11\textwidth}   
         \centering
         \includegraphics[width=\textwidth, page=5]{figure_assets/segment_qual.pdf}
     \end{subfigure}     
     \hfill
     % Fourth Row
     \hfill
     \begin{subfigure}[b]{0.11\textwidth}  
         \centering
         \includegraphics[width=\textwidth, page=3]{figure_assets/segment_qual.pdf}
         \caption*{GT}
     \end{subfigure}     
     \begin{subfigure}[b]{0.11\textwidth}   
         \centering
         \includegraphics[width=\textwidth, page=9]{figure_assets/segment_qual.pdf}
         \caption*{$I_{\text{seg}}$}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.11\textwidth}  
         \centering
         \includegraphics[width=\textwidth, page=12]{figure_assets/segment_qual.pdf}
         \caption*{$I_{\text{seg}}$ \& $M_{\text{seg}}$}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.11\textwidth}  
         \centering
         \includegraphics[width=\textwidth, page=6]{figure_assets/segment_qual.pdf}
         \caption*{$M_{\text{seg}}$ (Ours)}  
     \end{subfigure}   
     \caption{
    Qualitative ablations on types of images for segmentation.
}
     \label{fig:segment_qual}
\end{figure}


==> sec/supp_list.tex <==
% SILog Metric 수식 추가

% Rendered Handpose 내용 옮기기
% Rendered handpose dataset에서 MDE model Global, Segment affine transform 결과 측정
% Rendered handpose dataset 그림 수정 (배경의 depth값 날리고, hand에 해당하는 depth값으로 colormap 수정해보기, 지금은 hand는 완전 푸른색 단색으로 나와서 문제됨)
% ClearGrasp와 Rendered handpose에서 iMAE나 iRMSE 뽑을 수 있나? supple에 표 만드면 나쁘지 않을듯

% Model Agnosticism across MDE models에 DepthAnythingV2와 비교했는데 (Table S4), 우리가 main paper에서 비교했던 Metric3D나 Unidepth로 비교해 볼 수 있나? Depthanything v2와 비교한 결과는 큰 의미가 없을거 같아서

% Segment-wise affine transform과 StarryGazer(Ours)에서 Segment-wise SILog average 구할 수 있나? global SILog하고 같이 비교해서 설명할 수 있으면 좋을듯


% (정말 시간되면) ICCV Reviewer3가 이야기했던 dataset 하나 더 실험 추가

----

%

==> tables/Adaptation.tex <==
\begin{table}[h!]
    \centering
    \small
    \setlength{\tabcolsep}{3pt} % tweak this if you need it narrower

    \begin{tabular}{c|cc}
        \toprule
        Method & MAE~(m) $\downarrow$ & RMSE~(m) $\downarrow$  \\
        \midrule
        NLSPN w/o adaptation & 0.389 & 0.703  \\
        NLSPN+ProxyTTA       & \textbf{0.124} & 0.241   \\
        NLSPN+Ours           & 0.153 & \textbf{0.222} \\
        \bottomrule
    \end{tabular}

    \caption{Evaluation of our method's performance as a test-time adaptation approach compared to other adaptation methods.}
    \label{fig:adap} % (you might want \label{tab:adap}, but this is optional)
    \vspace{-2mm}
\end{table}

==> tables/ClearGrasp.tex <==
\begin{table*}[t]
\centering
\caption{Quantitative results on the ClearGrasp Dataset~\cite{ClearGrasp}.}
\resizebox{\textwidth}{!}{%
    \begin{tabular}{c|c|c|c|c|c|c|c}
        \toprule
        Supervision & Method & MAE~(m) $\downarrow$ & RMSE~(m) $\downarrow$ & $\delta_{\substack{\text{1.05}}} \uparrow$ & $\delta_{\substack{\text{1.10}}}  \uparrow$ & $\delta_{\substack{\text{1.25}}} \uparrow$ & Rel $\downarrow$  \\
        \midrule
        \multirow{6}{*}{Supervised Learning}
        & DenseDepth~\cite{DenseDepth} & $0.260$ & $0.270$ & $0.187$ & $0.343$ & $0.583$ & $0.428$ \\
        & DeepCompletion~\cite{DeepCompletion} & $0.045$ & $0.054$ & $0.445$ & $0.678$ & $0.958$ & $0.081$ \\
        & NLSPN~\cite{NLSPN} & $0.106$ & $0.132$ & $0.163$ & $0.321$ & $0.648$ & $0.239$ \\
        & ClearGrasp~\cite{ClearGrasp} & $0.038$ & $0.044$ & $0.414$ & $0.792$ & $0.973$ & $0.074$ \\
        & LocalImplicit~\cite{LocalImplicit} & $0.034$ & $0.041$ & $0.527$ & $0.794$ & $0.981$ & $0.063$ \\
        & TranspareNet~\cite{TranspareNet} & $0.027$ & $\textbf{0.032}$ & $0.608$ & $0.805$ & $0.982$ & $\textbf{0.052}$ \\
        \midrule
        Self-Supervised Learning 
        & Ours  & $\textbf{0.025}$ & $0.062$ & $\textbf{0.946}$ & $\textbf{0.976}$ & $\textbf{0.989}$ & $0.082$ \\
        \bottomrule
    \end{tabular}
}
\label{tab:ClearGrasp}
\end{table*}


==> tables/MDE_KITTIDC.tex <==
% \begin{table}[h]
% \centering
% \caption{Quantitative comparison with MDE methods on KITTI DC dataset.}
% \resizebox{0.8\textwidth}{!}{%
%     \begin{tabular}{c|c|c|c}
%         \toprule
%         Method  & RMSE & $\delta_{\substack{\text{1.25}}} \uparrow$ & Rel $\downarrow$  \\
%         \midrule
%         \multirow{6}{*}{Depth Estimation}
%         ZoeDepth~\cite{zoedepth} & $2.281$  & $0.971$ & $0.053$ \\
%         ZeroDepth~\cite{towards_zeroshot}  & $2.087$  & $0.968$ & $0.057$ \\
%         NeWCRFs~\cite{newcrfs} & $2.129$ & $0.974$ & $0.052$ \\
%         IEBins~\cite{IEBins} & $2.011$  & $0.978$ & $0.050$ \\
%         Metric3D~\cite{Metric3D}  & $1.766$  & $0.989$ & $0.039$ \\
%         DepthAnything~\cite{DepthAnything}  & $1.896$  & $0.982$ & $0.046$ \\
%         DepthAnything V2~\cite{depth_anything_v2} & $1.861$ & $0.983$ & $0.045$ \\
%         \midrule
%         Ours  & $\textbf{1.061}$  & $\textbf{0.995}$ & $\textbf{0.039}$ \\
%         \bottomrule
%     \end{tabular}
% }
% \label{tab:MDE_KITTI}
% \end{table}

==> tables/MDE_nyu.tex <==
% \begin{table}[h]
% \centering
% \caption{Quantitative comparison with MDE methods on NYU Depth V2 dataset.}
% \resizebox{0.8\textwidth}{!}{%
%     \begin{tabular}{c|c|c|c}
%         \toprule
%         Method & RMSE $\downarrow$  & $\delta_{\substack{\text{1.25}}} \uparrow$ & Rel $\downarrow$  \\
%         \midrule
%         ZoeDepth~\cite{zoedepth} &   $0.277$  & $0.953$ & $0.077$ \\
%         ZeroDepth~\cite{towards_zeroshot} &  $0.269$  & $0.954$ & $0.074$ \\
%         NeWCRFs~\cite{newcrfs}  & $0.334$ & $0.922$ & $0.095$\\
%         IEBins~\cite{IEBins}&  $0.314$  & $0.936$ & $0.087$ \\
%         Metric3D~\cite{Metric3D} &  $0.187$  & $0.987$ & $0.045$ \\
%         DepthAnything~\cite{DepthAnything} &  $0.206$  & $0.984$ & $0.056$ \\
%         DepthAnything V2~\cite{depth_anything_v2} &  $0.206$  & $0.984$ & $0.056$ \\
%         \midrule
%         Ours   & $\textbf{0.171}$  & $\textbf{0.999}$ & $\textbf{0.039}$ \\
%         \bottomrule
%     \end{tabular}
% }

% \label{tab:MDE_NYU}
% \end{table}

==> tables/Noise_test.tex <==
\begin{table}[h]
\centering

\label{table:noise_comparison}
\begin{tabular}{@{}c|ccccc@{}}
\toprule
Noise Level ($\sigma$) & MAE~(m) $\downarrow$ & RMSE~(m) $\downarrow$ & \\ \midrule
0   & 0.100 & 0.171 \\
0.001 & 0.103 & 0.180  \\
0.01 & 0.104 & 0.181 \\
0.1 & 0.114 & 0.188 \\

\bottomrule
\end{tabular}
\caption{Performance comparison with Different Levels of Gaussian Noise.}
\label{tab:noise_test}
\end{table}
    

==> tables/RHP.tex <==
\begin{wraptable}{r}{0.45\textwidth}
\centering
\resizebox{0.45\textwidth}{!}{%
    \begin{tabular}{c|cc}
    \toprule
                       Dataset & \multicolumn{2}{c}{ClearGrasp} & \multicolumn{2}{c}{Rendered Handpose} \\
    \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5}
                        Method & MAE~(m)$_\downarrow$  & RMSE~(m)$_\downarrow$  & MAE~(m)$_\downarrow$  & RMSE~(m)$_\downarrow$  \\
    \midrule
    DenseDepth~\cite{DenseDepth} & $0.260$ & $0.270$ & $-$ & $-$ \\
    DeepCompletion~\cite{DeepCompletion} & $0.045$ & $0.054$ & $-$ & $-$  \\
    NLSPN~\cite{NLSPN} & $0.106$ & $0.132$ & $0.485$ & $0.563$  \\
    CompletionFormer ~\cite{CompletionFormer} & $-$ & $-$ & $0.443$ & $0.524$ \\
    ClearGrasp~\cite{ClearGrasp} & $0.038$ & $0.044$ & $-$ & $-$  \\
    LocalImplicit~\cite{LocalImplicit} & $0.034$ & $0.041$ & $-$ & $-$  \\
    TranspareNet~\cite{TranspareNet} & $0.027$ & $\textbf{0.032}$ & $-$ & $-$ \\
    Depth Prompting~\cite{park2024depth} & 0.462 & 0.530 & 0.700  & 0.797             \\

    \midrule
    UniDepth V2~\cite{unidepth}  & 0.296 & 0.311 & 0.407 & 0.526              \\
    Metric3D V2~\cite{metric3dv2}   & 0.230 & 0.261 & 0.479 & 0.564             \\
    \midrule
    Ours       & \textbf{0.025}  & 0.062 & \textbf{0.352}  & \textbf{0.408}             \\
    \bottomrule
    \end{tabular}
}
\caption{Quantitative comparison on out-of-domain datasets.}
\label{tab:ood}
\vspace{-2mm}
\end{wraptable}

% ClearGrasp  비교
% Metric3D RMSE: 0.261  MAE: 0.230 
% DepthPrompting RMSE: 0.5301  MAE: 0.4621
% UniDepth RMSE: 0.311 MAE: 0.296

%RHD 비교
% Metric3D RMSE: 0.564   MAE: 0.479
% DepthPrompting RMSE: 0.797  MAE: 0.700 
% UniDepth RMSE: 0.526 MAE: 0.407


==> tables/Supervised_KITTI.tex <==
\begin{table}[h]
\centering
\caption{Quantitative Comparison with Supervised Depth Completion Methods on KITTI DC.}
\resizebox{0.45\textwidth}{!}{%
    \begin{tabular}{c|cc}
        \toprule
        Method & MAE $\downarrow$ & RMSE $\downarrow$ \\
        \midrule
        CSPN~\cite{CSPN} & $0.279$ & $1.019$ \\
        DeepLiDAR~\cite{DeepLiDAR} &  $0.226$ & $0.758$ \\
        GuideNet~\cite{GuideNet} &  $0.218$ & $0.736$ \\
        NLSPN~\cite{NLSPN} & $0.199$ & $0.741$ \\
        PENet~\cite{PENet} & $0.210$ & $0.730$ \\
        ACMNet~\cite{AdaContext} &  $0.206$ & $0.744$ \\
        TWISE~\cite{TWISE} & $0.195$ & $0.840$ \\
        RigNet~\cite{RigNet} & $0.203$ & $0.712$ \\
        GuideFormer~\cite{guideformer} & $0.207$ & $0.721$ \\  
        DySPN~\cite{DySPN} &  $0.192$ & $0.709$ \\ 
        CompletionFormer~\cite{CompletionFormer} & $0.203$ & $0.708$ \\  \
        SemAttNet~\cite{SemAttNet} & $0.205$ & $0.709$ \\  
        \midrule
        Ours & $0.242$ & $1.061$ \\
        \bottomrule
    \end{tabular}
}
\label{tab:Sup_KITTI}
\end{table}

==> tables/Supervised_NYU.tex <==
\begin{table}[h!]
\centering
\caption{Quantitative Comparison with Supervised Depth Completion Methods on NYU Depth V2.}
\resizebox{0.45\textwidth}{!}{%
    \begin{tabular}{c|cc}
        \toprule
        Method & RMSE $\downarrow$ & Rel $\downarrow$  \\
        \midrule
        CSPN~\cite{CSPN} & $0.117$ & $0.016$ \\
        DeepLiDAR~\cite{DeepLiDAR} & $0.115$ & $0.022$  \\
        GuideNet~\cite{GuideNet} & $0.101$ & $0.015$ \\
        NLSPN~\cite{NLSPN} & $0.092$ & $0.012$  \\
        ACMNet~\cite{AdaContext} & $0.105$ & $0.015$  \\
        TWISE~\cite{TWISE} & $0.097$ & $0.013$  \\
        RigNet~\cite{RigNet} & $0.090$ & $0.012$  \\ 
        DySPN~\cite{DySPN} & $0.090$ & $0.012$ \\ 
        SpAgNet~\cite{SpAgNet} & $0.114$ & $0.015$\\  
        CompletionFormer~\cite{CompletionFormer} & $0.090$ & $0.012$  \\  
        \midrule
        Ours & $0.171$ & $0.039$\\
        \bottomrule
    \end{tabular}
}
\label{tab:Sup_NYU}
\end{table}

==> tables/ablations.tex <==
\begin{table}[h!]
    \centering
    % Subtable (a)
    \begin{subtable}[b]{\linewidth}
        \centering
        \resizebox{0.92\textwidth}{!}{
        \begin{tabular}{c|cc}
        \toprule
        Method & MAE~(m) $\downarrow$ & RMSE~(m) $\downarrow$  \\
        \midrule
        NLSPN w/o adaptation & $0.389$ & $0.703$  \\
        NLSPN+ProxyTTA & $\textbf{0.124}$ & $0.241$   \\
        NLSPN+Ours & $0.153$ & $\textbf{0.222}$ 
        \\
        \bottomrule
        \end{tabular}%
        }
        \caption{Quantitative comparison with a test-time adaptation method.}
        \label{fig:adap}
    \end{subtable}
    
    % Subtable (b)
    \begin{subtable}[b]{\linewidth}
        \centering
        \resizebox{0.92\textwidth}{!}{
        \begin{tabular}{@{}c|ccccc@{}}
        \toprule
        Method  & MAE~(m) $\downarrow$ & RMSE~(m) $\downarrow$\\ \midrule
        Global rescaling & 1.373 & 1.013\\
        Affine transformation & 0.574 & 0.664  \\
        Ours  & \textbf{0.100} &  \textbf{0.171} \\
        \bottomrule
        \end{tabular}}
        \caption{\small Comparison analysis for rescaling the relative depth map.}
        \label{fig:rescaling}
    \end{subtable}
    \caption{Analysis on test-time adaptation and relative depth map rescaling on NYU Depth V2 dataset.}
    \label{fig:ablations}
\vspace{-2mm}
\end{table}


==> tables/ablations_alpha_beta.tex <==
\begin{table}[t]
    \centering
    \caption{Ablations on different configurations of $\alpha$ and $\beta$.}
    \begin{tabular}{cc|cc}
    \toprule
    $\alpha$ & $\beta$ & {MAE~(m)$_\downarrow$} & {RMSE~(m)$_\downarrow$} \\
    \midrule
    Eq.~\ref{eq:rand_alpha} & 0 & 2.72 & 2.91 \\
    Eq.~\ref{eq:rand_alpha} & Eq.~\ref{eq:alpha_beta} & 0.234 & 0.326 \\
    % 1 & 0 & 2.10 & 2.27 \\
    \midrule
    Eq.~\ref{eq:alpha_beta} & Eq.~\ref{eq:alpha_beta} & \textbf{0.100} & \textbf{0.171} \\
    \bottomrule
    \end{tabular}
\label{tab:ablation_alpha_beta}
\end{table}

% \textbf{} & \textbf{MAE} & \textbf{RMSE} \\
% \midrule
% $\alpha_k \sim \mathcal{U}(\min(D_s), \max(D_s))$, $\beta = 0$ & 2.72 & 2.91 \\
% $\alpha = 1$, $\beta = 0$ & 2.10 & 2.27 \\
% $\alpha_k \sim \mathcal{U}(\min(D_s), \max(D_s))$, random $\beta$ & 0.234 & 0.326 \\
% Ours & \textbf{0.100} & \textbf{0.171} \\

==> tables/ablations_rescaling.tex <==

\begin{table}[h!]
    \caption{Comparison with relative depth map rescaling.}
    \resizebox{0.47\textwidth}{!}{
    \begin{tabular}{@{}c|ccccc@{}}
        \toprule
        Method  & MAE~(m)$_\downarrow$ & RMSE~(m)$_\downarrow$\\
        \midrule
        Global affine transformation & 0.334 & 0.434\\
        Segment-wise affine transformation & 0.225 & 0.512  \\
        \midrule
        Ours  & \textbf{0.100} &  \textbf{0.171} \\
        \bottomrule
    \end{tabular}}
    \label{tab:rescaling}
\end{table}

==> tables/loss_ablation.tex <==
% Define \cmark and \crossmark commands
\newcommand\chkmark[1][]{%
  \tikz[scale=0.4,#1]{\fill(0,.35) -- (.25,0) -- (1,.7) -- (.25,.15) -- cycle;}%
}

\newcommand\crossmark[1][]{%
  \tikz[scale=0.4,#1]{
    \fill(0,0)--(0.1,0) .. controls (0.5,0.4) .. (1,0.7)--(0.9,0.7) ..  controls (0.5,0.5) ..(0,0.1) --cycle;
    \fill(1,0.1)--(0.9,0.1) .. controls (0.5,0.3) .. (0,0.7)--(0.1,0.7) .. controls (0.5,0.4) ..(1,0.2) --cycle;
  }%
}

\begin{wraptable}{r}{0.4\textwidth}
\centering
\caption{Effect of $\mathcal{L}^{ssim}$ and noise addition.}
\small % Change the font size here
\resizebox{0.4\textwidth}{!}{%
    \begin{tabular}{lcccc}
                \toprule
                $\mathcal{L}^{mse}$ & $\mathcal{L}^{ssim}$ & $Noise$ & {MAE~(m)$_\downarrow$} & {RMSE~(m)$_\downarrow$} \\
                \midrule
                \chkmark[blue] & \crossmark[red] & \crossmark[red] & $0.132$ & $0.212$ \\
                \chkmark[blue] & \chkmark[blue] & \crossmark[red] & $0.118$ & $0.190$ \\
                \chkmark[blue] & \crossmark[red] & \chkmark[blue] & $0.112$ & $0.192$ \\       
                \midrule
                \chkmark[blue] & \chkmark[blue] & \chkmark[blue] & $\textbf{0.100}$ & $\textbf{0.171}$ \\
                \bottomrule
            \end{tabular}}
\normalsize
\label{fig:ablation_loss}
\end{wraptable}

==> tables/mde_type.tex <==
\begin{table}[h!]
\centering
\small
\vspace{-2mm}
\resizebox{0.2\textwidth}{!}{%
    \begin{tabular}{c|c|c}
        \toprule
        Source of Relative Depth & MAE $\downarrow$  & RMSE $\downarrow$  \\
        \midrule
        NewCRF~\textcolor{blue}{[48]} &  $0.118$  & $0.186$  \\
        ZoeDepth~\textcolor{blue}{[1]} &   $0.092$  & $0.171$  \\
        GT depth &  $0.210$  & $0.256$  \\
        \bottomrule
    \end{tabular}
}
\vspace{-2mm}
\label{tab:ablation_mde}
\end{table}
